Graph Signal Sampling for Inductive One-Bit Matrix Completion: a Closed-form Solution

Inductive one-bit matrix completion is motivated by modern applications such as recommender systems, where new users would appear at test stage with the ratings consisting of only ones and no zeros. We propose a unified graph signal sampling framework which enjoys the benefits of graph signal analysis and processing. The key idea is to transform each user's ratings on the items to a function (signal) on the vertices of an item-item graph, then learn structural graph properties to recover the function from its values on certain vertices -- the problem of graph signal sampling. We propose a class of regularization functionals that takes into account discrete random label noise in the graph vertex domain, then develop the GS-IMC approach which biases the reconstruction towards functions that vary little between adjacent vertices for noise reduction. Theoretical result shows that accurate reconstructions can be achieved under mild conditions. For the online setting, we develop a Bayesian extension, i.e., BGS-IMC which considers continuous random Gaussian noise in the graph Fourier domain and builds upon a prediction-correction update algorithm to obtain the unbiased and minimum-variance reconstruction. Both GS-IMC and BGS-IMC have closed-form solutions and thus are highly scalable in large data. Experiments show that our methods achieve state-of-the-art performance on public benchmarks.

==> spectrum.tex <==

\begin{figure*}[tb!]
    \centerline{\includegraphics[width=.98\textwidth]{fig/Ampli_koubei.pdf}}
    \caption{\label{fig:vf_analysis}Spectrum analysis for static {\mname}, {\bname} and dynamic BERT4REC on the Koubei dataset. Compared to BERT4REC, the energy of {\mname} and {\bname} is concentrated on the low frequencies since the high-frequency functions are highly penalized during minimization.}
    \vskip -0.1in
\end{figure*}

\begin{wraptable}{r}{0.6\textwidth}
\begin{center}
\vspace{-18pt}
\caption{\label{tbl:seqsrec} Comparisons to neural sequential models for inductive top-N ranking on Koubei.}
\vspace{-3pt}
\resizebox{.58\textwidth}{!}{
	\begin{tabular}{!{\vrule width 1pt}l cccc !{\vrule width 1pt}} \noalign{\hrule height 1pt}
		\textbf{Model} &
		\textbf{BERT4REC} & 
		\textbf{SASREC} & 
		\textbf{GREC} &
		\textbf{\bname} \\\noalign{\hrule height 1pt}
		\textbf{H@10} &
		0.23760 & 0.23015 & 
		0.22405 & \textbf{0.24390} \\
		\textbf{H@50} &
		0.32385 & 0.30500 & 
		0.30065 & \textbf{0.32545} \\
		\textbf{H@100} &
		\textbf{0.35965} & 0.34735 & 
		0.34350 & 0.35345 
		\\\noalign{\hrule height 1pt}
		\textbf{N@10} &
		\textbf{0.18822} & 0.18496 & 
		0.18118 & 0.17854 \\
		\textbf{N@50} &
		\textbf{0.20663} & 0.20137 &
		0.19816 & 0.19680 \\
		\textbf{N@100} &
		\textbf{0.21402} & 0.20819 &
		0.20583 & 0.20134 
		\\\noalign{\hrule height 1pt}
		\textbf{Runtime} &
		89 min & 37 min &
		27 min & \textbf{83 sec}
		\\\noalign{\hrule height 1pt}
\end{tabular}}\end{center}
\vspace{-16pt}
\end{wraptable}
\subsection{Spectrum Analysis and Discussion with Sequential Models}\label{sec:specseqn}
Finally, we also compare with recent sequential recommendation models, including transformer-based SASREC \citep{kang2018self}, BERT-based BERT4REC \citep{sun2019bert4rec} and causal convolutional neural networks based GREC \citep{yuan2020future}. The embedding size is set to $256$ and the optimal hyper-parameters are searched by grid. Each of the model is configured using the same parameters provided by the original paper i.e., two attention blocks with one head for SASREC, three attention blocks with eight heads for BERT4REC and six dilated CNNs with degrees $1, 2, 2, 4, 4, 8$ for GREC. 
Table \ref{tbl:seqsrec} presents HR and NDCG on Koubei for inductive top-N ranking. Note that {\bname} only accepts the most recent behavior to update the obsolete states for incremental learning, whereas SASREC, BERT4REC and GREC focus on modeling the dynamic patterns within the entire sequence. Interestingly, our proposed static {\bname} model achieves comparable HR results to state-of-the-art sequential models, while consuming a small fraction of running time. From this viewpoint, {\bname} is more cost-effective than SASREC, BERT4REC and GREC.

To fully understand the performance gap in NDCG, we further study {\mname}, {\bname} and the best baseline BERT4REC in the graph spectral domain, where we limit the $\ell_2$ norm of each user's spectral signals to one and visualize their averaged values in Figure \ref{fig:vf_analysis}.  As expected, the energy of both {\mname} and {\bname} is concentrated on the low frequencies, since the high-frequency functions are highly penalized during minimization. Meanwhile, the Kalman filtering based inference in fact increases the energy of high-frequency functions. This bears a similarity with BERT4REC of which high-frequency functions are not constrained and can aggressively raise the rankings of unpopular items . This is the reason why BERT4REC and {\bname} have better accuracy in terms of NDCG than {\mname}.
